Bifurcations and dynamics in inertial focusing of particles in curved rectangular ducts

Particles suspended in fluid flow through a curved duct focus to stable equilibrium positions in the duct cross-section due to the balance of two dominant forces: (i) inertial lift force - arising from the inertia of the fluid, and (ii) secondary drag force - resulting from cross-sectional vortices induced by the curvature of the duct. Such particle focusing is exploited in various medical and industrial technologies aimed at separating particles by size. Using the theoretical model developed by Harding et al.~[7], we numerically investigate the dynamics of neutrally buoyant particles in fluid flow through curved ducts with rectangular cross-sections at low flow rates. We explore the rich bifurcations that take place in the particle equilibria as a function of three system parameters - particle size, duct bend radius and aspect ratio of the cross-section. We also explore the transient dynamics of particles as they focus to their equilibria by delineating the effects of these three parameters, as well as the initial location of the particle inside the cross-section, on the focusing dynamics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
